Constrained Optimization with Dynamic Bound-scaling for Effective NLPBackdoor Defense

We develop a novel optimization method for NLPbackdoor inversion. We leverage a dynamically reducing temperature coefficient in the softmax function to provide changing loss landscapes to the optimizer such that the process gradually focuses on the ground truth trigger, which is denoted as a one-hot value in a convex hull. Our method also features a temperature rollback mechanism to step away from local optimals, exploiting the observation that local optimals can be easily deter-mined in NLP trigger inversion (while not in general optimization). We evaluate the technique on over 1600 models (with roughly half of them having injected backdoors) on 3 prevailing NLP tasks, with 4 different backdoor attacks and 7 architectures. Our results show that the technique is able to effectively and efficiently detect and remove backdoors, outperforming 4 baseline methods.

==> Table/TrojAI_results.tex <==
\begin{table*}
\footnotesize
\centering
\caption{Evaluation Results on TrojAI Datasets}
\label{t:effectiveness}
%\setlength{\tabcolsep}{3pt}
\scalebox{0.7}{
\begin{tabular}{llrrrrrrrrrrrrrrrrrrrrrr}
\toprule
\multirow{2}{*}[-0.03in]{Task}  &\multirow{2}{*}[-0.03in]{Evaluation Set} & \multirow{2}{*}[-0.03in]{Arch} & \multicolumn{3}{c}{\textbf{CO}} & \multicolumn{1}{c}{} & \multicolumn{3}{c}{ASCC}  & \multicolumn{1}{c}{} & \multicolumn{3}{c}{UAT}  & \multicolumn{1}{c}{} & \multicolumn{3}{c}{T-miner*}  & \multicolumn{1}{c}{} & \multicolumn{3}{c}{Genetic} \\

\cmidrule{4-6} \cmidrule{8-10} \cmidrule{12-14} \cmidrule{16-18} \cmidrule{20-22}
 &  &   &  \multicolumn{1}{c}{\# models} & \multicolumn{1}{c}{Acc} &    \multicolumn{1}{c}{Time(s)} & \multicolumn{1}{c}{} &  \multicolumn{1}{c}{\# models} &  \multicolumn{1}{c}{Acc}  &  \multicolumn{1}{c}{Time(s)} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{\# models} &  \multicolumn{1}{c}{Acc}  &  \multicolumn{1}{c}{Time(s)} & \multicolumn{1}{c}{} &\multicolumn{1}{c}{\# models} &  \multicolumn{1}{c}{Acc}  &   \multicolumn{1}{c}{Time(s)} & \multicolumn{1}{c}{} &\multicolumn{1}{c}{\# models} &  \multicolumn{1}{c}{Acc}  &   \multicolumn{1}{c}{Time(s)} \\

\midrule
\multirow{4}{*}{SA} & \multirow{2}{*}{Train}    & DistilBERT        &24     &\textbf{0.958} &\textbf{162}         &   &24     &0.750  &140      &   &24     &0.958 &156    &   &24     &0.458  &2829    &   &24     &0.826  &1434\\
 &                                              & GPT               &24     &\textbf{0.958} &\textbf{238}         &   &24     &0.916  &259      &   &24     &0.750 &355    &   &24     &0.542  &3341    &   &24     &0.870 &1918\\
\cmidrule{2-22}
 & \multirow{2}{*}{Test}                        & DistilBERT        &240    &\textbf{0.951} &\textbf{164}         &   &240    &0.704  &156      &   &240    &0.936 &155    &   &100     &0.530  &2831   &   &120    &0.775  &1519\\
 &                                              & GPT               &240    &\textbf{0.958} &\textbf{240}         &   &240    &0.829  &262      &   &240    &0.772 &346    &   &100     &0.510  &3321   &   &120    &0.820  &1952\\
 \midrule
\multirow{8}{*}{NER} & \multirow{4}{*}{Train}   & BERT              &45     &\textbf{0.911} &\textbf{582}                   &   &45    &0.755 &702   &   &45  &0.911  &721   &   &-  &-  &-   &  &10\\
 &                                              & DistilBERT        &45     &\textbf{0.911} &\textbf{640}                    &   &45    &0.688 &721   &   &45  &0.755 &810   &   &-  &-  &-    &  &10\\
 &                                              & RoBERTa        &45     &\textbf{0.933} &\textbf{595}                       &   &45    &0.644 &668   &   &45  &0.933 &701   &   &-  &-  &-    &  &10\\
 &                                              & MobileBERT        &45     &\textbf{0.911} &\textbf{502}                    &   &45    &0.866 &530   &   &45  &0.955 &623   &   &-  &-  &-    &  &10\\
\cmidrule{2-22}
 &\multirow{4}{*}{Test}                         & BERT              &90     &\textbf{0.933} &\textbf{601}                   &   &90    &0.733 &727   &   &90  &0.955 &725   &   &-  &-  &-    &  &20\\
 &                                              & DistilBERT        &90     &\textbf{0.888} &\textbf{652}                    &   &90    &0.544 &612   &   &90  &0.800 &821   &   &-  &-  &-    &  &20\\
 &                                              & RoBERTa        &90     &\textbf{0.933} &\textbf{622}                       &   &90    &0.644 &680   &   &90  &0.922 &702   &   &-  &-  &-    &  &20\\
 &                                              & MobileBERT        &90     &\textbf{0.911} &\textbf{519}                    &   &90    &0.822 &540   &   &90  &0.911 &625   &   &-  &-  &-    &  &20\\
 \midrule
\multirow{6}{*}{QA} & \multirow{3}{*}{Train}    & RoBERTa           &40     &\textbf{0.975} &\textbf{685}                   &  &40     &0.850 &635   &   &40  &0.900  &767 &   &-  &-  &-  &  &20\\
 &                                              & Deepset           &40     &\textbf{1.000} &\textbf{646}                    &  &40     &0.825 &658   &   &40  &0.925  &820 &   &-  &-  &-  &  &20\\
 &                                              & Google Electra    &40     &\textbf{0.950} &\textbf{260}                   &   &40     &0.750 &226   &   &40  &0.850  &258 &   &-  &-  &-  &  &20\\ 
\cmidrule{2-22}
 & \multirow{3}{*}{Test}                        & RoBERTa           &120    &\textbf{0.908} &\textbf{692}                    &  &120     &0.701 &658   &   &120  &0.800  &766 &   &-  &-  &- &  &40\\
 &                                              & Deepset           &120    &\textbf{0.908} &\textbf{642}                     &  &120     &0.725 &711   &   &120  &0.798  &812 &   &-  &-  &- &  &40\\
 &                                              & Google Electra    &120    &\textbf{0.900} &\textbf{262}                     &  &120     &0.658 &321   &   &120  &0.750  &262 &   &-  &-  &- &  &40\\ 
\bottomrule
\multicolumn{19}{l}{*Due to T-miner running too slow, we test T-miner on randomly sampled 100 models on R5-test and R6-test dataset} \\

\end{tabular}
}
\end{table*}
